A New Sensing 5'-->3' Watson-Crick Automata Concept

Watson-Crick (WK) finite automata are working on a Watson-Crick tape, that is, on a DNA molecule. Therefore, it has two reading heads. While in traditional WK automata both heads read the whole input in the same physical direction, in 5'->3' WK automata the heads start from the two extremes and read the input in opposite direction. In sensing 5'->3' WK automata the process on the input is finished when the heads meet. Since the heads of a WK automaton may read longer strings in a transition, in previous models a so-called sensing parameter took care for the proper meeting of the heads (not allowing to read the same positions of the input in the last step). In this paper, a new model is investigated, which works without the sensing parameter (it is done by an appropriate change of the concept of configuration). Consequently, the accepted language classes of the variants are also changed. Various hierarchy results are proven in the paper.

==> eptcsdata.tex <==
\providecommand{\firstpage}{195}
\providecommand{\publicationstatus}{E. Csuhaj-Varj\'u, P. D\"om\"osi, Gy. Vaszil (Eds.): 15th International \\ Conference on Automata and Formal Languages (AFL 2017)\\
EPTCS 252, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.252.19}{10.4204/EPTCS.252.19}}
\pdfoutput=1

